PaMIR: Parametric Model-Conditioned Implicit Representation for Image-based Human Reconstruction

Modeling 3D humans accurately and robustly from a single image is very challenging, and the key for such an ill-posed problem is the 3D representation of the human models. To overcome the limitations of regular 3D representations, we propose Parametric Model-Conditioned Implicit Representation (PaMIR), which combines the parametric body model with the free-form deep implicit function. In our PaMIR-based reconstruction framework, a novel deep neural network is proposed to regularize the free-form deep implicit function using the semantic features of the parametric model, which improves the generalization ability under the scenarios of challenging poses and various clothing topologies. Moreover, a novel depth-ambiguity-aware training loss is further integrated to resolve depth ambiguities and enable successful surface detail reconstruction with imperfect body reference. Finally, we propose a body reference optimization method to improve the parametric model estimation accuracy and to enhance the consistency between the parametric model and the implicit function. With the PaMIR representation, our framework can be easily extended to multi-image input scenarios without the need of multi-camera calibration and pose synchronization. Experimental results demonstrate that our method achieves state-of-the-art performance for image-based 3D human reconstruction in the cases of challenging poses and clothing types.

==> 1.intro-old.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:intro}}
\IEEEPARstart{I}{mage-based} parsing of human bodies is a popular topic in computer graphics and 3D vision. 
Among all the tasks of image-based human parsing, recovering 3D human from a single RGB image attracts more and more interests given its wide applications in VR/AR content creation, image and video editing, telepresence and virtual dressing. 
However, as an ill-posed problem, recovering 3D humans from a single RGB image is very challenging due to the variations of body shapes, poses, clothing types, and lighting conditions. 

Benefiting from the huge progress of deep learning techniques, recent studies have tried to address these challenges using learning-based methods\cite{BodyNet,SiCloPe2019,HMD2019,tex2shape2019,Zheng2019DeepHuman,MouldingHumans2019,pifuSHNMKL19}. According to their 3D representation, these methods can be roughly classified into two categories: parametric methods and non-parametric methods. Parametric methods like HMD\cite{HMD2019} and Tex2Shape\cite{tex2shape2019} utilize a statistical body template model (e.g., SMPL\cite{SMPL:2015}) as the geometrical prior and learn to deform the template according to the silhouette and the shading information. 
However, the low dimensional parametric model limits the performance when handling different clothing types(e.g., long dresses and skirts). 
%The main challenge of parametric methods is that they are inherently incapable to handle loose clothes like dresses and skirts. 
Non-parametric methods use various free-form representations, including voxel grids\cite{BodyNet}, silhouettes\cite{SiCloPe2019}, implicit fields\cite{pifuSHNMKL19} or depth maps\cite{MouldingHumans2019}, to represent 3D human models. 
Although being able to describe arbitrary clothes, current non-parametric methods still suffer from challenging poses and self-occlusions due to the lack of semantic information and insufficient training data. 

Recently, DeepHuman\cite{Zheng2019DeepHuman} pioneered the combination of the parametric SMPL model and the non-parametric volumetric representation, and demonstrates robust reconstruction for challenging poses and diverse garments. 
However, it struggles to recover high-quality geometric details due to the resolution limitation of the regular occupancy volume. More importantly, combining the parametric SMPL model with the non-parametric representation raises a crucial problem: 
%how to deal with the inconsistency between the input SMPL model and the RGB input? 
how can we obtain accurate SMPL model estimation given a single image at testing time? 
In DeepHuman, the input SMPL models are estimated using learning-based methods and/or optimization-based methods. As a result, the quality of the final reconstruction  results heavily depends on the consistency between the image and the estimated SMPL model: misalignment between them will lead to erroneous results. 
Although the recent years have witness a renaissance in the context of single-image body shape estimation\cite{Bogo:ECCV:2016,omran2018NBF,HMR,kolotouros2019cmr,liang2019shapeaware,xu2019denserac}, we observed that there is still an \emph{accuracy gap} between the training and testing stages: during training, we can obtain well-aligned SMPL models for the training data by fitting the SMPL template to the high quality scans, while for testing, the SMPL estimations provided by the state-of-the-art single-image methods\cite{HMR,kolotouros2019cmr} still cannot align with the keypoints or the silhouettes as perfectly as the SMPL models in the training dataset. 
%Moreover, even if the estimated SMPL perfectly aligns with 2D image representation, it is impossible to guarantee the alignment along the depth axis due to depth ambiguities.

As a result, the neural network trained with the ground-truth image-SMPL pairs cannot generalize well to the testing images which have no ground-truth SMPL annotations. 
A simple solution is to replace the ground-truth SMPL models with the predicted ones while still using the ground-truth surface scans for training supervision, preventing the network from heavy dependence on accurate SMPL annotations. 
However, due to depth ambiguities, it is impossible to guarantee well alignments between the predicted SMPL models and the ground-truth scans along the depth axis. 
Consequently, by doing so we are forcing the networks to make ``correct'' geometry inference given a ``wrong'' SMPL reference along the depth axis, which will generate even worse results.

%Recent studies have tried to address these challenges using techniques based on silhouette estimation\cite{SiCloPe2019}, template deformation\cite{HMD2019,tex2shape2019}, depth estimation\cite{MouldingHumans2019}, volumetric reconstruction\cite{BodyNet,Zheng2019DeepHuman} and implicit functions\cite{PIFUSHNMKL19}. Unfortunately, none of them can achieve general, accurate and robust reconstruction from a single image. 

% \begin{figure}
% 	\begin{center}
% 		\includegraphics[width=1.0\linewidth]{teaser}
% 	\end{center}
% 	\caption{Example results reconstructed by our method from a single image. }
% 	\label{fig:teaser}
% \end{figure}


   
%For single-image human reconstruction, the inner body template and the outer surface are mutually beneficial: on one hand, body template estimation can serve as a reference for surface reconstruction\cite{Zheng2019DeepHuman}; on the other hand, as the surface reconstruction is the back-projection of the image feature into 3D space, it can also be used to constrain the body prediction result from the input image. 
%Based on this observation, we propose to jointly reconstruct the geometry surface as well as the underlying body shape from a single image and address the issue of the accuracy gap in three aspects: network architecture, loss definition and top-down optimization. For network architecture, we first propose PIVOIF, an novel implicit function that is conditioned on both the pixel-aligned image feature and the voxel-aligned body shape feature. To convert 


To overcome the accuracy gap between ground truth training data and inaccurate testing input, in this paper, we propose a novel hybrid 3D representation by combining \emph{Parametric And Implicit Representation}, dubbed PAIR, which incorporates parametric SMPL model and free-form deep implicit function. We further propose a new depth-ambiguity-aware training loss, and a body reference optimization method. 
%we incorporate the parametric SMPL model with the non-parametric implicit representation and address the issue of accuracy gap in three aspects:

\begin{itemize}%[leftmargin=*]
    % \setlength{\itemsep}{0pt}
    % \setlength{\parsep}{0pt}
    % \setlength{\parskip}{0pt}
    
%    \item \textbf{Network Architecture.} To condition the implicit field on the SMPL prediction, we propose a novel implicit function that converts an image feature map and the corresponding SMPL feature volume into an implicit surface. The 3D feature volume is encoded from the predicted SMPL mesh using our novel \emph{neural voxelization layer}. Thanks to its differentiability, the supervision signal on surface reconstruction can be back propagated to the body estimation network and consequently improves its estimation accuracy.  
%    We propose \emph{Parametric And Implicit Representation}, dubbed PAIR, which incorporates parametric SMPL model and free-form deep implicit function. 
    
\item \textbf{PAIR.} 
    Our PAIR representation has the ability to condition the implicit field on the SMPL prediction, which is realized by a novel network architecture to convert an image feature map and the corresponding SMPL feature volume into an implicit surface representation. The SMPL feature volume is directly encoded from the SMPL prediction provided by GraphCMR\cite{kolotouros2019cmr}, and serves as a soft constraint for handling challenging poses and/or self-occlusions. 
    Moreover, in PAIR, it is not necessary for the initial SMPL prediction to be highly accurate (which is usually the case for single RGB SMPL estimation), a roughly correct estimation on the xy-plane is enough to avoid the negative impact of inaccurate SMPL prediction on the final reconstruction.
    %Our PAIR representation only requires the SMPL model to be roughly correct on xy-plane, avoiding the negative impact of inaccurate SMPL prediction. 

    \item \textbf{Training Losses.} 
    To close the accuracy gap of SMPL prediction, we use the predicted SMPL models at both the training and the testing stages. Since depth ambiguities are inevitable in single image setups, it is unpractical to require the estimated bodies to align perfectly with the ground-truth human scans in the depth direction. Therefore, in order to make the network to be more robust against the inaccurate body reference along the depth direction, instead of using a naive reconstruction loss, we propose a \emph{depth-ambiguity-aware reconstruction loss} that adaptively adjusts the reconstruction supervision based on the current SMPL estimation while respecting 2D image observations. 
    
    %Furthermore, we introduce an efficient \emph{body fitting loss} that penalizes the misalignment between the estimated SMPL model and the predicted implicit surface. These two losses are complementary for closing the accuracy gap: the depth-ambiguity-aware reconstruction loss alleviates the requirement of perfect SMPL predictions, while the body fitting loss serves as an additional supervision to improve the accuracy of SMPL estimation. 
    
    \item \textbf{Body Reference Optimization.} 
    We also propose an \emph{instance-level body reference optimization} method for testing process to further refine the body reference. Our optimization method directly utilizes the network itself as well as its outputs to construct an efficient energy function for body fitting. The optimization further alleviates the error caused by the inaccurate initial SMPL estimation, and consequently closing the accuracy gap of SMPL estimation between training and testing. 
\end{itemize}

% [Need modification: better transition]
% To address these challenges, we propose to jointly reconstruction the body shape and surface geometry from a single image. Our key observation is that for single-image human reconstruction, the inner body template and the outer surface are mutually beneficial: on one hand, surface reconstruction can benefit from body template estimation as proven in DeepHuman\cite{Zheng2019DeepHuman}; on the other hand, since ...... 

Overall, the underlying body template and the outer surface are mutually beneficial in our method: on one hand, through the depth-ambiguity-aware reconstruction loss, the estimated body template serves as a 3D reference for outer surface reconstruction; on the other hand, the deep implicit function network is also used to optimize the body reference by minimizing the body fitting error. 
Furthermore, thanks to the usage of the common underlying SMPL model as body reference, our PAIR representation implicitly builds a correspondence relationship across different models. As a result, our method can be easily extended to multi-image setups like multi-view inputs or video inputs without calibration and synchronization. 
Experiments show that our method is able to reconstruct high-quality human models with various body shapes, poses and clothes, and outperforms state-of-the-art methods in terms of accuracy, robustness and generalization capability. 


% In summary, our method includes the following contributions:
% \begin{itemize}
%     \item 
% \end{itemize}

%which will make the network totally ignore the SMPL input. (Actually in practice we found that this naive solution will result into unstable training and worse results than original PIFu\cite{pifuSHNMKL19}. )

%Although achieving impressive results, these methods all have their limitations: silhouette-based methods like \cite{SiCloPe2019} suffer from lack of details and view inconsistency, model deformation based methods\cite{HMD2019,tex2shape2019} are unable to handle loose clothes; and depth-based methods like \cite{MouldingHumans2019} struggle with self occlusion. 

%Among all the afore-mentioned approaches, PIFu\cite{pifuSHNMKL19} and DeepHuman\cite{Zheng2019DeepHuman} are the most promising ones, and they have surprisingly complementary features. PIFu\cite{pifuSHNMKL19} achieves high-quality reconstruction by using a continuous implicit function as geometrical representation, but their method cannot generalize to challenging poses because it only uses 2D image features to infer the ``thichness'' along z-axis of the body, which varies widely for some body parts and cannot be easily determined from the 2D observation. 
%The reason for its incapability of generalization is that the implicit function in PIFu is only conditioned on pixel-aligned 2D image features and z-coordinates; unfortunately, for some body parts like arms, the  ``thichness'' along z-axis varies widely from pose to pose and cannot be easily determined from the 2D observation. (See Fig.\ref{} for an example. ) 
%despite suffering from the limited resolution of volumetric representation, 
%In contrast, DeepHuman\cite{Zheng2019DeepHuman} can generalize to different poses and is able to output plausible reconstruction results even under the scenarios of challenging poses and/or extreme occlusions. The robustness of DeepHuman is based on a valuable insight: parametric body template estimation (e.g., SMPL\cite{SMPL:2015}) can provide 3D body shape and pose information and thus resolves depth ambiguities for the network, leaving the neural network an easier task of adding the clothing layers. 

%Based on the above observations, it is a fair assumption that by combining PIFu and DeepHuman one can obtain an approach that outputs high-quality results and has robust performance. However, we empirically found that the performance of such an approach heavily relies on the accuracy of the input body template. While we can easily obtain accurate parametric body shapes for training data (because we have ground-truth meshes), for testing we have to rely on other external methods like\cite{HMR,kolotouros2019cmr,omran2018NBF} to estimate the body shape and pose from the single input image.  Unfortunately, current methods for single-image body inference sometimes provide unsatisfactory estimation (e.g., bent legs for standing poses, distant hands from the body for akimbo gestures) due to the shortage of accurate ground-truth labeling in available real-world datasets\cite{UnitethePeople2017}. Therefore, directly using the estimation provided by these methods in some cases is unhelpful, if not harmful, for the accuracy of reconstruction results. 

% For single-image human reconstruction, the inner body template and the outer surface are mutually beneficial: on one hand, surface reconstruction can benefit from body template estimation as proven in DeepHuman\cite{Zheng2019DeepHuman}; on the other hand, since .....
% On the basic of this insight, we go beyond simply combining PIFu with DeepHuman and propose ???(), an end-to-end framework for the reconstruction of high-quality human mesh as well as parametric body shape. Our proposed approach contains the following contributions:
% \begin{itemize}
%     \item We propose an implicit function that is conditioned on both 2D pixel-aligned features and 3D voxel-aligned features
%     \item We propose an neural voxelization layer to connect GraphCMR and PIFu
%     \item We propose 
% \end{itemize}



%Idea: combine them together: first contribution: spatially-aligned function

%Reliance on SMPL estimation: second contribution: neural voxelization + end-to-end training + SMPL-in-mesh loss

%Plausible SMPL without inaccurate depth: third contribution: adaptive sampling

%adaptive sampling: SMPL---> mesh
%SMPL-in-mesh loss: mesh---> SMPL


% Contribution:
% \begin{itemize}
%     \item SMPL + mesh, reasonable alignment relationship, insensitive to SMPL depth ambiguity
%     \item better SMPL estimation, robust mesh reconstruction
%     \item Adaptive samples
%     \item SMPL-in-mesh loss
%     \item Neural voxelization layer which enables end-to-end training
%     \item spatially aligned feature to improve the robustness
% \end{itemize}
